Session Types for the Transport Layer: Towards an Implementation of TCP

Session types are a typing discipline used to formally describe communication-driven applications with the aim of fewer errors and easier debugging later into the life cycle of the software. Protocols at the transport layer such as TCP, UDP, and QUIC underpin most of the communication on the modern Internet and affect billions of end-users. The transport layer has different requirements and constraints compared to the application layer resulting in different requirements for verification. Despite this, to our best knowledge, no work shows the application of session types at the transport layer. In this work, we discuss how multiparty session types (MPST) can be applied to implement the TCP protocol. We develop an MPST-based implementation of a subset of a TCP server in Rust and test its interoperability against the Linux TCP stack. Our results highlight the differences in assumptions between session type theory and the way transport layer protocols are usually implemented. This work is the first step towards bringing session types into the transport layer.

==> eptcsdata.tex <==
\providecommand{\firstpage}{22}
\providecommand{\publicationstatus}{D. Costa, R. Hu (Eds.): Programming Language Approaches to\\ Concurrency and Communication-cEntric Software 2024 (PLACES'24)\\
EPTCS 401, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{https://dx.doi.org/10.4204/EPTCS.401.3}{10.4204/EPTCS.401.3}}
\pdfoutput=1

